Run2Survive: A Decision-theoretic Approach to Algorithm Selection based on Survival Analysis

Algorithm selection (AS) deals with the automatic selection of an algorithm from a fixed set of candidate algorithms most suitable for a specific instance of an algorithmic problem class, where "suitability" often refers to an algorithm's runtime. Due to possibly extremely long runtimes of candidate algorithms, training data for algorithm selection models is usually generated under time constraints in the sense that not all algorithms are run to completion on all instances. Thus, training data usually comprises censored information, as the true runtime of algorithms timed out remains unknown. However, many standard AS approaches are not able to handle such information in a proper way. On the other side, survival analysis (SA) naturally supports censored data and offers appropriate ways to use such data for learning distributional models of algorithm runtime, as we demonstrate in this work. We leverage such models as a basis of a sophisticated decision-theoretic approach to algorithm selection, which we dub Run2Survive. Moreover, taking advantage of a framework of this kind, we advocate a risk-averse approach to algorithm selection, in which the avoidance of a timeout is given high priority. In an extensive experimental study with the standard benchmark ASlib, our approach is shown to be highly competitive and in many cases even superior to state-of-the-art AS approaches.

==> [ACML] Survival Analysis for Algorithm Selection/figures/scatter_asf.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	xmin=0,
	ymax=100,
	xmax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=AutoSurvivalForest,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.3619704970840113  0.678307188167013  ISAC*LIKE
0.1896392797062668  0.37057365073897225  ISAC*LIKE
0.4885481210537633  0.5816052568612295  ISAC*LIKE
0.2856889145572622  0.5228777822385304  ISAC*LIKE
2.574075453233949  25.005638168808908  ISAC*LIKE
0.3354411269837004  0.633979482712966  ISAC*LIKE
1.0116773331890154  0.7481160175040764  ISAC*LIKE
0.18842793802823307  0.3261541897619934  ISAC*LIKE
0.4133490247933328  0.6389066027778655  ISAC*LIKE
0.11745385536136335  0.5812831273846424  ISAC*LIKE
0.7405963051347608  0.9934845900321652  ISAC*LIKE
0.11066999294849617  0.3413740797208365  ISAC*LIKE
0.3668520683585846  0.7624399041017158  ISAC*LIKE
0.2690839315836035  0.4861309454590885  ISAC*LIKE
0.41599062484434457  1.00515320448719  ISAC*LIKE
0.9195871559690609  1.0863970459350147  ISAC*LIKE
0.6841207546775827  0.9530686135732818  ISAC*LIKE
0.9387152543158956  0.9781483425377416  ISAC*LIKE
0.4598447342846818  0.7013855838560397  ISAC*LIKE
8.19537516141494  3.0343187770427167  ISAC*LIKE
0.4660467725106746  0.6258720210231875  ISAC*LIKE
0.1975875599291004  0.8326084433409955  ISAC*LIKE
2.3536212972027872  4.635001851451788  ISAC*LIKE
0.5717033062529501  1.0160971015557598  ISAC*LIKE
0.7224238489198411  0.9580734424707004  ISAC*LIKE
0.30079348539086304  0.6527293218054211  ISAC*LIKE
0.3619704970840113  0.3727068040715841  PERALGORITHMREGRESSOR
0.1896392797062668  0.3561022296987444  PERALGORITHMREGRESSOR
0.4885481210537633  0.6127153109711706  PERALGORITHMREGRESSOR
0.2856889145572622  0.3549811173547622  PERALGORITHMREGRESSOR
2.574075453233949  2.390995304730814  PERALGORITHMREGRESSOR
0.3354411269837004  0.326774931576485  PERALGORITHMREGRESSOR
1.0116773331890154  0.7245332418766008  PERALGORITHMREGRESSOR
0.18842793802823307  0.2171794958650953  PERALGORITHMREGRESSOR
0.4133490247933328  0.4521638388413735  PERALGORITHMREGRESSOR
0.11745385536136335  0.1365715014720295  PERALGORITHMREGRESSOR
0.7405963051347608  0.7798023256886788  PERALGORITHMREGRESSOR
0.11066999294849617  0.125197658996884  PERALGORITHMREGRESSOR
0.3668520683585846  0.3900456945793733  PERALGORITHMREGRESSOR
0.2690839315836035  0.2565890812097911  PERALGORITHMREGRESSOR
0.41599062484434457  0.4220812771207481  PERALGORITHMREGRESSOR
0.9195871559690609  1.0369553794225423  PERALGORITHMREGRESSOR
0.6841207546775827  0.6089795737986103  PERALGORITHMREGRESSOR
0.9387152543158956  0.909550971459662  PERALGORITHMREGRESSOR
0.4598447342846818  0.5092849527012576  PERALGORITHMREGRESSOR
8.19537516141494  10.046493826664182  PERALGORITHMREGRESSOR
0.4660467725106746  0.6703583113478012  PERALGORITHMREGRESSOR
0.1975875599291004  0.17656354601663074  PERALGORITHMREGRESSOR
2.3536212972027872  4.018239865130491  PERALGORITHMREGRESSOR
0.5717033062529501  0.6461771054988412  PERALGORITHMREGRESSOR
0.7224238489198411  0.868896361056391  PERALGORITHMREGRESSOR
0.30079348539086304  0.3173743198219577  PERALGORITHMREGRESSOR
0.3619704970840113  0.4157567289098781  SUNNY*LIKE
0.1896392797062668  0.3420544115873054  SUNNY*LIKE
0.4885481210537633  0.5102692334591704  SUNNY*LIKE
0.2856889145572622  0.38778415792083704  SUNNY*LIKE
2.574075453233949  11.024140970070023  SUNNY*LIKE
0.3354411269837004  0.4199871970968848  SUNNY*LIKE
1.0116773331890154  1.0144015263116142  SUNNY*LIKE
0.18842793802823307  0.2342363871867101  SUNNY*LIKE
0.4133490247933328  0.472568787142205  SUNNY*LIKE
0.11745385536136335  0.13413782935635393  SUNNY*LIKE
0.7405963051347608  0.8264661375466948  SUNNY*LIKE
0.11066999294849617  0.13519036320762598  SUNNY*LIKE
0.3668520683585846  0.28487456563991603  SUNNY*LIKE
0.2690839315836035  0.27891490037641364  SUNNY*LIKE
0.41599062484434457  0.24347647329399344  SUNNY*LIKE
0.9195871559690609  1.1005666866952357  SUNNY*LIKE
0.6841207546775827  0.7690655151737142  SUNNY*LIKE
0.9387152543158956  0.9877233823201352  SUNNY*LIKE
0.4598447342846818  0.5190616864954294  SUNNY*LIKE
8.19537516141494  8.895331064742077  SUNNY*LIKE
0.4660467725106746  0.5613114268682801  SUNNY*LIKE
0.1975875599291004  0.24146530135189825  SUNNY*LIKE
2.3536212972027872  11.525693770202654  SUNNY*LIKE
0.5717033062529501  0.4872517183107655  SUNNY*LIKE
0.7224238489198411  0.8194358754277964  SUNNY*LIKE
0.30079348539086304  0.19807847047517213  SUNNY*LIKE
0.3619704970840113  0.4025668486665903  SATZILLA'11*LIKE
0.1896392797062668  0.29502449425618205  SATZILLA'11*LIKE
0.4885481210537633  0.6201886117590589  SATZILLA'11*LIKE
0.2856889145572622  0.34692854380740423  SATZILLA'11*LIKE
2.574075453233949  40.47124191666446  SATZILLA'11*LIKE
0.3354411269837004  0.2821401701836627  SATZILLA'11*LIKE
1.0116773331890154  0.7281512246422769  SATZILLA'11*LIKE
0.18842793802823307  0.15409546878934588  SATZILLA'11*LIKE
0.4133490247933328  0.56949283393721  SATZILLA'11*LIKE
0.11745385536136335  0.36224385773615614  SATZILLA'11*LIKE
0.7405963051347608  0.6409090386556566  SATZILLA'11*LIKE
0.11066999294849617  0.2072072017576949  SATZILLA'11*LIKE
0.3668520683585846  0.4662401081022946  SATZILLA'11*LIKE
0.2690839315836035  0.2383579026242359  SATZILLA'11*LIKE
0.41599062484434457  0.4013072777852713  SATZILLA'11*LIKE
0.9195871559690609  0.8918135633190942  SATZILLA'11*LIKE
0.6841207546775827  0.7909236746193591  SATZILLA'11*LIKE
0.9387152543158956  0.8511395055215155  SATZILLA'11*LIKE
0.4598447342846818  0.40416828060962395  SATZILLA'11*LIKE
8.19537516141494  9.040038521329254  SATZILLA'11*LIKE
0.4660467725106746  0.4382131452252581  SATZILLA'11*LIKE
0.1975875599291004  0.17632633083365565  SATZILLA'11*LIKE
2.3536212972027872  4.728210093497262  SATZILLA'11*LIKE
0.5717033062529501  0.5884760955910446  SATZILLA'11*LIKE
0.7224238489198411  0.8541750308083232  SATZILLA'11*LIKE
0.30079348539086304  0.4688268909116234  SATZILLA'11*LIKE
0.3619704970840113  0.3661192613385954  MULTICLASSSELECTOR
0.1896392797062668  0.7816601153543972  MULTICLASSSELECTOR
0.4885481210537633  0.6765204702029799  MULTICLASSSELECTOR
0.2856889145572622  0.6292123480351777  MULTICLASSSELECTOR
2.574075453233949  59.70167589543316  MULTICLASSSELECTOR
0.3354411269837004  0.4125744853023916  MULTICLASSSELECTOR
1.0116773331890154  0.8613737468472333  MULTICLASSSELECTOR
0.18842793802823307  0.3333403316545537  MULTICLASSSELECTOR
0.4133490247933328  0.8372401386776829  MULTICLASSSELECTOR
0.11745385536136335  0.17342325582160995  MULTICLASSSELECTOR
0.7405963051347608  0.9426330676164544  MULTICLASSSELECTOR
0.11066999294849617  0.31028969535327755  MULTICLASSSELECTOR
0.3668520683585846  0.841125297437588  MULTICLASSSELECTOR
0.2690839315836035  0.3707292833375948  MULTICLASSSELECTOR
0.41599062484434457  1.2440671401636696  MULTICLASSSELECTOR
0.9195871559690609  5.316655519540719  MULTICLASSSELECTOR
0.6841207546775827  0.75823175512707  MULTICLASSSELECTOR
0.9387152543158956  0.9358700154462076  MULTICLASSSELECTOR
0.4598447342846818  0.6089544785846619  MULTICLASSSELECTOR
8.19537516141494  9.745508035939428  MULTICLASSSELECTOR
0.4660467725106746  0.5741456751186104  MULTICLASSSELECTOR
0.1975875599291004  0.31481281763565755  MULTICLASSSELECTOR
2.3536212972027872  8.762749094703938  MULTICLASSSELECTOR
0.5717033062529501  1.1773932311669637  MULTICLASSSELECTOR
0.7224238489198411  0.9938409073890452  MULTICLASSSELECTOR
0.30079348539086304  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
	    (0.2,0.2)
	    (0.3,0.3)
	    (0.4,0.4)
	    (0.5,0.5)
	    (0.6,0.6)
	    (0.7,0.7)
	    (0.8,0.8)
	    (0.9,0.9)
	    (1,1)
	    (1.5,1.5)
		(2,2)
		(3,3)
		(4,4)
		(5,5)
		(6,6)
		(7,7)
		(8,8)
		(10,10)
		(100,100)
	};
	\end{axis}
\end{tikzpicture}

==> [ACML] Survival Analysis for Algorithm Selection/figures/scatter_esf.tex <==
\begin{tikzpicture}
	\begin{semilogyaxis}[%
	xmin=0,
	xmax=100,
	ymax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=ExpectationSurvivalForest,
	log ticks with fixed point,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.36631947541879695  0.678307188167013  ISAC*LIKE
0.2592832599339565  0.37057365073897225  ISAC*LIKE
0.4744089449595796  0.5816052568612295  ISAC*LIKE
0.3007385914842758  0.5228777822385304  ISAC*LIKE
2.5766243051276114  25.005638168808908  ISAC*LIKE
0.34902915573329063  0.633979482712966  ISAC*LIKE
1.0106928871325442  0.7481160175040764  ISAC*LIKE
0.1934212219443083  0.3261541897619934  ISAC*LIKE
0.4083934578602521  0.6389066027778655  ISAC*LIKE
0.13551202514865812  0.5812831273846424  ISAC*LIKE
0.7322069990826827  0.9934845900321652  ISAC*LIKE
0.11120358643431127  0.3413740797208365  ISAC*LIKE
0.4596011123631822  0.7624399041017158  ISAC*LIKE
0.2690613866762786  0.4861309454590885  ISAC*LIKE
0.3891742445877905  1.00515320448719  ISAC*LIKE
0.9953247242720892  1.0863970459350147  ISAC*LIKE
0.6573188045299808  0.9530686135732818  ISAC*LIKE
0.9733953124318652  0.9781483425377416  ISAC*LIKE
0.4603411780387689  0.7013855838560397  ISAC*LIKE
4.531596581362732  3.0343187770427167  ISAC*LIKE
0.5147341205889762  0.6258720210231875  ISAC*LIKE
0.20438456695669927  0.8326084433409955  ISAC*LIKE
2.400257262697644  4.635001851451788  ISAC*LIKE
0.5696449903581586  1.0160971015557598  ISAC*LIKE
0.7227773541996839  0.9580734424707004  ISAC*LIKE
0.3007482452133336  0.6527293218054211  ISAC*LIKE
0.36631947541879695  0.3727068040715841  PERALGORITHMREGRESSOR
0.2592832599339565  0.3561022296987444  PERALGORITHMREGRESSOR
0.4744089449595796  0.6127153109711706  PERALGORITHMREGRESSOR
0.3007385914842758  0.3549811173547622  PERALGORITHMREGRESSOR
2.5766243051276114  2.390995304730814  PERALGORITHMREGRESSOR
0.34902915573329063  0.326774931576485  PERALGORITHMREGRESSOR
1.0106928871325442  0.7245332418766008  PERALGORITHMREGRESSOR
0.1934212219443083  0.2171794958650953  PERALGORITHMREGRESSOR
0.4083934578602521  0.4521638388413735  PERALGORITHMREGRESSOR
0.13551202514865812  0.1365715014720295  PERALGORITHMREGRESSOR
0.7322069990826827  0.7798023256886788  PERALGORITHMREGRESSOR
0.11120358643431127  0.125197658996884  PERALGORITHMREGRESSOR
0.4596011123631822  0.3900456945793733  PERALGORITHMREGRESSOR
0.2690613866762786  0.2565890812097911  PERALGORITHMREGRESSOR
0.3891742445877905  0.4220812771207481  PERALGORITHMREGRESSOR
0.9953247242720892  1.0369553794225423  PERALGORITHMREGRESSOR
0.6573188045299808  0.6089795737986103  PERALGORITHMREGRESSOR
0.9733953124318652  0.909550971459662  PERALGORITHMREGRESSOR
0.4603411780387689  0.5092849527012576  PERALGORITHMREGRESSOR
4.531596581362732  10.046493826664182  PERALGORITHMREGRESSOR
0.5147341205889762  0.6703583113478012  PERALGORITHMREGRESSOR
0.20438456695669927  0.17656354601663074  PERALGORITHMREGRESSOR
2.400257262697644  4.018239865130491  PERALGORITHMREGRESSOR
0.5696449903581586  0.6461771054988412  PERALGORITHMREGRESSOR
0.7227773541996839  0.868896361056391  PERALGORITHMREGRESSOR
0.3007482452133336  0.3173743198219577  PERALGORITHMREGRESSOR
0.36631947541879695  0.4157567289098781  SUNNY*LIKE
0.2592832599339565  0.3420544115873054  SUNNY*LIKE
0.4744089449595796  0.5102692334591704  SUNNY*LIKE
0.3007385914842758  0.38778415792083704  SUNNY*LIKE
2.5766243051276114  11.024140970070023  SUNNY*LIKE
0.34902915573329063  0.4199871970968848  SUNNY*LIKE
1.0106928871325442  1.0144015263116142  SUNNY*LIKE
0.1934212219443083  0.2342363871867101  SUNNY*LIKE
0.4083934578602521  0.472568787142205  SUNNY*LIKE
0.13551202514865812  0.13413782935635393  SUNNY*LIKE
0.7322069990826827  0.8264661375466948  SUNNY*LIKE
0.11120358643431127  0.13519036320762598  SUNNY*LIKE
0.4596011123631822  0.28487456563991603  SUNNY*LIKE
0.2690613866762786  0.27891490037641364  SUNNY*LIKE
0.3891742445877905  0.24347647329399344  SUNNY*LIKE
0.9953247242720892  1.1005666866952357  SUNNY*LIKE
0.6573188045299808  0.7690655151737142  SUNNY*LIKE
0.9733953124318652  0.9877233823201352  SUNNY*LIKE
0.4603411780387689  0.5190616864954294  SUNNY*LIKE
4.531596581362732  8.895331064742077  SUNNY*LIKE
0.5147341205889762  0.5613114268682801  SUNNY*LIKE
0.20438456695669927  0.24146530135189825  SUNNY*LIKE
2.400257262697644  11.525693770202654  SUNNY*LIKE
0.5696449903581586  0.4872517183107655  SUNNY*LIKE
0.7227773541996839  0.8194358754277964  SUNNY*LIKE
0.3007482452133336  0.19807847047517213  SUNNY*LIKE
0.36631947541879695  0.4025668486665903  SATZILLA'11*LIKE
0.2592832599339565  0.29502449425618205  SATZILLA'11*LIKE
0.4744089449595796  0.6201886117590589  SATZILLA'11*LIKE
0.3007385914842758  0.34692854380740423  SATZILLA'11*LIKE
2.5766243051276114  40.47124191666446  SATZILLA'11*LIKE
0.34902915573329063  0.2821401701836627  SATZILLA'11*LIKE
1.0106928871325442  0.7281512246422769  SATZILLA'11*LIKE
0.1934212219443083  0.15409546878934588  SATZILLA'11*LIKE
0.4083934578602521  0.56949283393721  SATZILLA'11*LIKE
0.13551202514865812  0.36224385773615614  SATZILLA'11*LIKE
0.7322069990826827  0.6409090386556566  SATZILLA'11*LIKE
0.11120358643431127  0.2072072017576949  SATZILLA'11*LIKE
0.4596011123631822  0.4662401081022946  SATZILLA'11*LIKE
0.2690613866762786  0.2383579026242359  SATZILLA'11*LIKE
0.3891742445877905  0.4013072777852713  SATZILLA'11*LIKE
0.9953247242720892  0.8918135633190942  SATZILLA'11*LIKE
0.6573188045299808  0.7909236746193591  SATZILLA'11*LIKE
0.9733953124318652  0.8511395055215155  SATZILLA'11*LIKE
0.4603411780387689  0.40416828060962395  SATZILLA'11*LIKE
4.531596581362732  9.040038521329254  SATZILLA'11*LIKE
0.5147341205889762  0.4382131452252581  SATZILLA'11*LIKE
0.20438456695669927  0.17632633083365565  SATZILLA'11*LIKE
2.400257262697644  4.728210093497262  SATZILLA'11*LIKE
0.5696449903581586  0.5884760955910446  SATZILLA'11*LIKE
0.7227773541996839  0.8541750308083232  SATZILLA'11*LIKE
0.3007482452133336  0.4688268909116234  SATZILLA'11*LIKE
0.36631947541879695  0.3661192613385954  MULTICLASSSELECTOR
0.2592832599339565  0.7816601153543972  MULTICLASSSELECTOR
0.4744089449595796  0.6765204702029799  MULTICLASSSELECTOR
0.3007385914842758  0.6292123480351777  MULTICLASSSELECTOR
2.5766243051276114  59.70167589543316  MULTICLASSSELECTOR
0.34902915573329063  0.4125744853023916  MULTICLASSSELECTOR
1.0106928871325442  0.8613737468472333  MULTICLASSSELECTOR
0.1934212219443083  0.3333403316545537  MULTICLASSSELECTOR
0.4083934578602521  0.8372401386776829  MULTICLASSSELECTOR
0.13551202514865812  0.17342325582160995  MULTICLASSSELECTOR
0.7322069990826827  0.9426330676164544  MULTICLASSSELECTOR
0.11120358643431127  0.31028969535327755  MULTICLASSSELECTOR
0.4596011123631822  0.841125297437588  MULTICLASSSELECTOR
0.2690613866762786  0.3707292833375948  MULTICLASSSELECTOR
0.3891742445877905  1.2440671401636696  MULTICLASSSELECTOR
0.9953247242720892  5.316655519540719  MULTICLASSSELECTOR
0.6573188045299808  0.75823175512707  MULTICLASSSELECTOR
0.9733953124318652  0.9358700154462076  MULTICLASSSELECTOR
0.4603411780387689  0.6089544785846619  MULTICLASSSELECTOR
4.531596581362732  9.745508035939428  MULTICLASSSELECTOR
0.5147341205889762  0.5741456751186104  MULTICLASSSELECTOR
0.20438456695669927  0.31481281763565755  MULTICLASSSELECTOR
2.400257262697644  8.762749094703938  MULTICLASSSELECTOR
0.5696449903581586  1.1773932311669637  MULTICLASSSELECTOR
0.7227773541996839  0.9938409073890452  MULTICLASSSELECTOR
0.3007482452133336  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
		(100,100)
	};
	\end{semilogyaxis}
\end{tikzpicture}

==> [ACML] Survival Analysis for Algorithm Selection/figures/scatter_gssf.tex <==
\begin{tikzpicture}
	\begin{semilogyaxis}[%
	xmin=0,
	xmax=100,
	ymax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=nPAR10 GridSearchSurvivalForest,
	ylabel=nPAR10 Baseline,
	log ticks with fixed point,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.3595703063406438  0.678307188167013  ISAC*LIKE
0.24237898483093134  0.37057365073897225  ISAC*LIKE
0.4885539473876691  0.5816052568612295  ISAC*LIKE
0.3037088355194861  0.5228777822385304  ISAC*LIKE
2.577448890275856  25.005638168808908  ISAC*LIKE
0.3355424548592121  0.633979482712966  ISAC*LIKE
0.94590081392888  0.7481160175040764  ISAC*LIKE
0.19233936774392985  0.3261541897619934  ISAC*LIKE
0.4156346977057006  0.6389066027778655  ISAC*LIKE
0.11009614002362557  0.5812831273846424  ISAC*LIKE
0.7268223371245681  0.9934845900321652  ISAC*LIKE
0.11390021428666255  0.3413740797208365  ISAC*LIKE
0.36938359885355504  0.7624399041017158  ISAC*LIKE
0.2691410807256949  0.4861309454590885  ISAC*LIKE
0.414190330188758  1.00515320448719  ISAC*LIKE
0.9561134869872088  1.0863970459350147  ISAC*LIKE
0.7036296835341059  0.9530686135732818  ISAC*LIKE
0.8960219654197135  0.9781483425377416  ISAC*LIKE
0.5603193890982832  0.7013855838560397  ISAC*LIKE
4.393978741958076  3.0343187770427167  ISAC*LIKE
0.3854524480930018  0.6258720210231875  ISAC*LIKE
0.20539526376817102  0.8326084433409955  ISAC*LIKE
2.3858604230905835  4.635001851451788  ISAC*LIKE
0.5761557175705883  1.0160971015557598  ISAC*LIKE
0.7399812539598516  0.9580734424707004  ISAC*LIKE
0.3363421530290565  0.6527293218054211  ISAC*LIKE
0.3595703063406438  0.3727068040715841  PERALGORITHMREGRESSOR
0.24237898483093134  0.3561022296987444  PERALGORITHMREGRESSOR
0.4885539473876691  0.6127153109711706  PERALGORITHMREGRESSOR
0.3037088355194861  0.3549811173547622  PERALGORITHMREGRESSOR
2.577448890275856  2.390995304730814  PERALGORITHMREGRESSOR
0.3355424548592121  0.326774931576485  PERALGORITHMREGRESSOR
0.94590081392888  0.7245332418766008  PERALGORITHMREGRESSOR
0.19233936774392985  0.2171794958650953  PERALGORITHMREGRESSOR
0.4156346977057006  0.4521638388413735  PERALGORITHMREGRESSOR
0.11009614002362557  0.1365715014720295  PERALGORITHMREGRESSOR
0.7268223371245681  0.7798023256886788  PERALGORITHMREGRESSOR
0.11390021428666255  0.125197658996884  PERALGORITHMREGRESSOR
0.36938359885355504  0.3900456945793733  PERALGORITHMREGRESSOR
0.2691410807256949  0.2565890812097911  PERALGORITHMREGRESSOR
0.414190330188758  0.4220812771207481  PERALGORITHMREGRESSOR
0.9561134869872088  1.0369553794225423  PERALGORITHMREGRESSOR
0.7036296835341059  0.6089795737986103  PERALGORITHMREGRESSOR
0.8960219654197135  0.909550971459662  PERALGORITHMREGRESSOR
0.5603193890982832  0.5092849527012576  PERALGORITHMREGRESSOR
4.393978741958076  10.046493826664182  PERALGORITHMREGRESSOR
0.3854524480930018  0.6703583113478012  PERALGORITHMREGRESSOR
0.20539526376817102  0.17656354601663074  PERALGORITHMREGRESSOR
2.3858604230905835  4.018239865130491  PERALGORITHMREGRESSOR
0.5761557175705883  0.6461771054988412  PERALGORITHMREGRESSOR
0.7399812539598516  0.868896361056391  PERALGORITHMREGRESSOR
0.3363421530290565  0.3173743198219577  PERALGORITHMREGRESSOR
0.3595703063406438  0.4157567289098781  SUNNY*LIKE
0.24237898483093134  0.3420544115873054  SUNNY*LIKE
0.4885539473876691  0.5102692334591704  SUNNY*LIKE
0.3037088355194861  0.38778415792083704  SUNNY*LIKE
2.577448890275856  11.024140970070023  SUNNY*LIKE
0.3355424548592121  0.4199871970968848  SUNNY*LIKE
0.94590081392888  1.0144015263116142  SUNNY*LIKE
0.19233936774392985  0.2342363871867101  SUNNY*LIKE
0.4156346977057006  0.472568787142205  SUNNY*LIKE
0.11009614002362557  0.13413782935635393  SUNNY*LIKE
0.7268223371245681  0.8264661375466948  SUNNY*LIKE
0.11390021428666255  0.13519036320762598  SUNNY*LIKE
0.36938359885355504  0.28487456563991603  SUNNY*LIKE
0.2691410807256949  0.27891490037641364  SUNNY*LIKE
0.414190330188758  0.24347647329399344  SUNNY*LIKE
0.9561134869872088  1.1005666866952357  SUNNY*LIKE
0.7036296835341059  0.7690655151737142  SUNNY*LIKE
0.8960219654197135  0.9877233823201352  SUNNY*LIKE
0.5603193890982832  0.5190616864954294  SUNNY*LIKE
4.393978741958076  8.895331064742077  SUNNY*LIKE
0.3854524480930018  0.5613114268682801  SUNNY*LIKE
0.20539526376817102  0.24146530135189825  SUNNY*LIKE
2.3858604230905835  11.525693770202654  SUNNY*LIKE
0.5761557175705883  0.4872517183107655  SUNNY*LIKE
0.7399812539598516  0.8194358754277964  SUNNY*LIKE
0.3363421530290565  0.19807847047517213  SUNNY*LIKE
0.3595703063406438  0.4025668486665903  SATZILLA'11*LIKE
0.24237898483093134  0.29502449425618205  SATZILLA'11*LIKE
0.4885539473876691  0.6201886117590589  SATZILLA'11*LIKE
0.3037088355194861  0.34692854380740423  SATZILLA'11*LIKE
2.577448890275856  40.47124191666446  SATZILLA'11*LIKE
0.3355424548592121  0.2821401701836627  SATZILLA'11*LIKE
0.94590081392888  0.7281512246422769  SATZILLA'11*LIKE
0.19233936774392985  0.15409546878934588  SATZILLA'11*LIKE
0.4156346977057006  0.56949283393721  SATZILLA'11*LIKE
0.11009614002362557  0.36224385773615614  SATZILLA'11*LIKE
0.7268223371245681  0.6409090386556566  SATZILLA'11*LIKE
0.11390021428666255  0.2072072017576949  SATZILLA'11*LIKE
0.36938359885355504  0.4662401081022946  SATZILLA'11*LIKE
0.2691410807256949  0.2383579026242359  SATZILLA'11*LIKE
0.414190330188758  0.4013072777852713  SATZILLA'11*LIKE
0.9561134869872088  0.8918135633190942  SATZILLA'11*LIKE
0.7036296835341059  0.7909236746193591  SATZILLA'11*LIKE
0.8960219654197135  0.8511395055215155  SATZILLA'11*LIKE
0.5603193890982832  0.40416828060962395  SATZILLA'11*LIKE
4.393978741958076  9.040038521329254  SATZILLA'11*LIKE
0.3854524480930018  0.4382131452252581  SATZILLA'11*LIKE
0.20539526376817102  0.17632633083365565  SATZILLA'11*LIKE
2.3858604230905835  4.728210093497262  SATZILLA'11*LIKE
0.5761557175705883  0.5884760955910446  SATZILLA'11*LIKE
0.7399812539598516  0.8541750308083232  SATZILLA'11*LIKE
0.3363421530290565  0.4688268909116234  SATZILLA'11*LIKE
0.3595703063406438  0.3661192613385954  MULTICLASSSELECTOR
0.24237898483093134  0.7816601153543972  MULTICLASSSELECTOR
0.4885539473876691  0.6765204702029799  MULTICLASSSELECTOR
0.3037088355194861  0.6292123480351777  MULTICLASSSELECTOR
2.577448890275856  59.70167589543316  MULTICLASSSELECTOR
0.3355424548592121  0.4125744853023916  MULTICLASSSELECTOR
0.94590081392888  0.8613737468472333  MULTICLASSSELECTOR
0.19233936774392985  0.3333403316545537  MULTICLASSSELECTOR
0.4156346977057006  0.8372401386776829  MULTICLASSSELECTOR
0.11009614002362557  0.17342325582160995  MULTICLASSSELECTOR
0.7268223371245681  0.9426330676164544  MULTICLASSSELECTOR
0.11390021428666255  0.31028969535327755  MULTICLASSSELECTOR
0.36938359885355504  0.841125297437588  MULTICLASSSELECTOR
0.2691410807256949  0.3707292833375948  MULTICLASSSELECTOR
0.414190330188758  1.2440671401636696  MULTICLASSSELECTOR
0.9561134869872088  5.316655519540719  MULTICLASSSELECTOR
0.7036296835341059  0.75823175512707  MULTICLASSSELECTOR
0.8960219654197135  0.9358700154462076  MULTICLASSSELECTOR
0.5603193890982832  0.6089544785846619  MULTICLASSSELECTOR
4.393978741958076  9.745508035939428  MULTICLASSSELECTOR
0.3854524480930018  0.5741456751186104  MULTICLASSSELECTOR
0.20539526376817102  0.31481281763565755  MULTICLASSSELECTOR
2.3858604230905835  8.762749094703938  MULTICLASSSELECTOR
0.5761557175705883  1.1773932311669637  MULTICLASSSELECTOR
0.7399812539598516  0.9938409073890452  MULTICLASSSELECTOR
0.3363421530290565  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
		(100,100)
	};
	\end{semilogyaxis}
\end{tikzpicture}

==> [ACML] Survival Analysis for Algorithm Selection/tables/aslib_table.tex <==
\begin{tabular}{lllllllllllllllllllllllllll}
\toprule
 & \rotatebox{90}{ASP-POTASSCO}  & \rotatebox{90}{BNSL-2016} & \rotatebox{90}{CPMP-2015} & \rotatebox{90}{CSP-2010} & \rotatebox{90}{CSP-MZN-2013} & \rotatebox{90}{CSP-Minizinc-Time-2016} & \rotatebox{90}{GRAPHS-2015} & \rotatebox{90}{MAXSAT-PMS-2016} & \rotatebox{90}{MAXSAT-WPMS-2016} & \rotatebox{90}{MAXSAT12-PMS} & \rotatebox{90}{MAXSAT15-PMS-INDU} & \rotatebox{90}{MIP-2016} & \rotatebox{90}{PROTEUS-2014} & \rotatebox{90}{QBF-2011} & \rotatebox{90}{QBF-2014} & \rotatebox{90}{QBF-2016} & \rotatebox{90}{SAT03-16\_INDU} & \rotatebox{90}{SAT11-HAND} & \rotatebox{90}{SAT11-INDU} & \rotatebox{90}{SAT11-RAND} & \rotatebox{90}{SAT12-ALL} & \rotatebox{90}{SAT12-HAND} & \rotatebox{90}{SAT12-INDU} & \rotatebox{90}{SAT12-RAND} & \rotatebox{90}{SAT15-INDU} & \rotatebox{90}{TSP-LION2015} \\
\midrule
\multicolumn{1}{l|}{\#I} &         1294 &      1179 &       527 &     2024 &         4642 &                    100 &        5725 &             601 &              630 &          876 &               601 &      218 &         4021 &     1368 &     1254 &      825 &          2000 &        296 &        300 &        600 &      1614 &        767 &       1167 &       1362 &        300 &         3106 \\
\multicolumn{1}{l|}{\#U} &           82 &         0 &         0 &      253 &          944 &                     17 &         117 &              45 &               89 &          129 &                44 &        0 &          456 &      314 &      241 &       55 &           269 &         77 &         47 &        108 &        20 &        229 &        209 &        322 &         17 &            0 \\
\multicolumn{1}{l|}{\#A} &           11 &         8 &         4 &        2 &           11 &                     20 &           7 &              19 &               18 &            6 &                29 &        5 &           22 &        5 &       14 &       24 &            10 &         15 &         18 &          9 &        31 &         31 &         31 &         31 &         28 &            4 \\
\multicolumn{1}{l|}{\#F} &          138 &        86 &        22 &       86 &          155 &                     95 &          35 &              37 &               37 &           37 &                37 &      143 &          198 &       46 &       46 &       46 &           483 &        115 &        115 &        115 &       115 &        115 &        115 &        115 &         54 &          122 \\
\multicolumn{1}{l|}{C}  &          600 &      7200 &      3600 &     5000 &         1800 &                   1200 &       1e+08 &            1800 &             1800 &         2100 &              1800 &     7200 &         3600 &     3600 &      900 &     1800 &          5000 &       5000 &       5000 &       5000 &      1200 &       1200 &       1200 &       1200 &       3600 &         3600 \\
\multicolumn{1}{l|}{\%C} &         20.1 &      28.1 &      27.6 &     19.6 &         70.2 &                     50 &           7.0 &            39.4 &             57.9 &         41.2 &              48.9 &       20 &         60.2 &     54.7 &     55.6 &     36.2 &          24.7 &       60.7 &       33.3 &       47.5 &      53.9 &       66.7 &       50.4 &       73.5 &       23.5 &          9.6 \\
\bottomrule
\end{tabular}


==> [ACML] Survival Analysis for Algorithm Selection/tables/normalized_table.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
& \parbox{2.3cm}{\centering Auto-\\ SurvivalForest} & \parbox{2.3cm}{\centering Expectation-\\ SurvivalForest} & \parbox{2.3cm}{\centering GridSearch-\\ SurvivalForest} &  \parbox{1.7cm}{\centering ISAC\\ *like} &  \parbox{2.0cm}{\centering MultiClass-\\ Selector} & \parbox{2.5cm}{\centering PerAlgorithm-\\ Regressor} &  \parbox{2.2cm}{\centering SATzilla'11\\ *like} &  \parbox{1.7cm}{\centering SUNNY\\ *like} \\
ASlib Scenario         &                     &                            &                           &            &                     &                        &                   &             \\
\midrule
ASP-POTASSCO           &            0.300793 &                   0.300748 &                  0.336342 &   0.652729 &            0.666993 &               0.320221 &          0.428925 &    0.172295 \\
BNSL-2016              &            0.197588 &                   0.204385 &                  0.205395 &   0.832608 &            0.314813 &               0.203520 &          0.197481 &    0.248938 \\
CPMP-2015              &            0.938715 &                   0.973395 &                  0.896022 &   0.978148 &            0.935870 &               0.882819 &          0.848480 &    1.050350 \\
CSP-2010               &            0.189639 &                   0.259283 &                  0.242379 &   0.370574 &            0.781660 &               0.365766 &          0.241954 &    0.402470 \\
CSP-MZN-2013           &            0.110670 &                   0.111204 &                  0.113900 &   0.341374 &            0.310290 &               0.135796 &          0.209275 &    0.125618 \\
CSP-Minizinc-Time-2016 &            0.459845 &                   0.460341 &                  0.560319 &   0.701386 &            0.608954 &               0.512432 &          0.502317 &    0.519079 \\
GRAPHS-2015            &            2.353621 &                   2.400257 &                  2.385860 &   4.635002 &            8.762749 &               5.960256 &          8.226409 &   11.525636 \\
MAXSAT-PMS-2016        &            0.571703 &                   0.569645 &                  0.576156 &   1.016097 &            1.177393 &               0.746590 &          0.591542 &    0.487082 \\
MAXSAT-WPMS-2016       &            0.366852 &                   0.459601 &                  0.369384 &   0.762440 &            0.841125 &               0.471578 &          0.429294 &    0.244580 \\
MAXSAT12-PMS           &            0.269084 &                   0.269061 &                  0.269141 &   0.486131 &            0.370729 &               0.302595 &          0.240272 &    0.278908 \\
MAXSAT15-PMS-INDU      &            0.415991 &                   0.389174 &                  0.414190 &   1.005153 &            1.244067 &               0.535373 &          0.430227 &    0.243505 \\
MIP-2016               &            8.195375 &                   4.531597 &                  4.393979 &   3.034319 &            9.745508 &              10.143470 &          9.662852 &    8.855730 \\
PROTEUS-2014           &            0.413349 &                   0.408393 &                  0.415635 &   0.638907 &            0.837240 &               0.450890 &          0.576535 &    0.473812 \\
QBF-2011               &            0.188428 &                   0.193421 &                  0.192339 &   0.326154 &            0.333340 &               0.195713 &          0.165905 &    0.220605 \\
QBF-2014               &            0.285689 &                   0.300739 &                  0.303709 &   0.522878 &            0.629212 &               0.334371 &          0.359988 &    0.397089 \\
QBF-2016               &            0.488548 &                   0.474409 &                  0.488554 &   0.581605 &            0.676520 &               0.626964 &          0.643596 &    0.510265 \\
SAT03-16\_INDU          &            0.722424 &                   0.722777 &                  0.739981 &   0.958073 &            0.993841 &               0.845725 &          0.882314 &    0.845817 \\
SAT11-HAND             &            0.466047 &                   0.514734 &                  0.385452 &   0.625872 &            0.574146 &               0.453943 &          0.453614 &    0.697061 \\
SAT11-INDU             &            0.684121 &                   0.657319 &                  0.703630 &   0.953069 &            0.758232 &               0.624086 &          0.842440 &    0.848683 \\
SAT11-RAND             &            0.117454 &                   0.135512 &                  0.110096 &   0.581283 &            0.173423 &               0.114355 &          0.374920 &    0.133021 \\
SAT12-ALL              &            0.361970 &                   0.366319 &                  0.359570 &   0.678307 &            0.366119 &               0.361825 &          0.428101 &    0.396569 \\
SAT12-HAND             &            0.335441 &                   0.349029 &                  0.335542 &   0.633979 &            0.412574 &               0.360927 &          0.305365 &    0.415547 \\
SAT12-INDU             &            0.740596 &                   0.732207 &                  0.726822 &   0.993485 &            0.942633 &               0.817029 &          0.642115 &    0.812497 \\
SAT12-RAND             &            0.919587 &                   0.995325 &                  0.956113 &   1.086397 &            5.316656 &               1.242140 &          0.916708 &    1.108742 \\
SAT15-INDU             &            1.011677 &                   1.010693 &                  0.945901 &   0.748116 &            0.861374 &               0.968517 &          0.804147 &    1.035853 \\
TSP-LION2015           &            2.574075 &                   2.576624 &                  2.577449 &  25.005638 &           59.701676 &               2.155110 &         41.317910 &   11.024178 \\
\bottomrule
\end{tabular}

==> [ACML] Survival Analysis for Algorithm Selection/tables/unsolved_table.tex <==
\begin{tabular}{l||rrr|rrrrr}
\toprule

 &  \parbox{2.3cm}{\centering Expectation-\\ SurvivalForest\\} &  \parbox{2.3cm}{\centering Auto-\\ SurvivalForest\\} &  \parbox{2.3cm}{\centering GridSearch-\\ SurvivalForest\\} &  \parbox{2.8cm}{\centering PerAlgorithm-\\Regressor\\(Runtime)} &  \parbox{2.0cm}{\centering MultiClass-\\Selector\\(Runtime)} &  \parbox{1.7cm}{\centering ISAC\\ *like\\(PAR10)} & \parbox{2.2cm}{\centering SATzilla'11\\ *like\\(Runtime)}  &  \parbox{1.7cm}{\centering SUNNY\\ *like\\(PAR10)} \\

\midrule
ASP-POTASSCO           &                        2.2 &                 2.2 &                       2.5 &                               2.4 &                            5.5 &                 5.3 &                          3.7 &                  1.3 \\
BNSL-2016              &                        2.4 &                 2.3 &                       2.4 &                               2.0 &                            3.8 &                10.0 &                          2.2 &                  3.0 \\
CPMP-2015              &                       15.8 &                15.2 &                      14.4 &                              14.4 &                           15.4 &                16.7 &                         14.0 &                 18.2 \\
CSP-2010               &                        0.6 &                 0.4 &                       0.5 &                               0.7 &                            1.5 &                 0.9 &                          0.6 &                  0.8 \\
CSP-MZN-2013           &                        3.5 &                 3.5 &                       3.6 &                               4.0 &                           10.6 &                11.6 &                          7.0 &                  4.0 \\
CSP-Minizinc-Time-2016 &                        8.7 &                 8.7 &                       9.9 &                               8.4 &                            8.4 &                 9.8 &                          7.4 &                  8.8 \\
GRAPHS-2015            &                        0.5 &                 0.5 &                       0.5 &                               0.6 &                            1.1 &                 0.7 &                          0.8 &                  0.5 \\
MAXSAT-PMS-2016        &                        2.5 &                 2.5 &                       2.5 &                               3.2 &                            5.6 &                 4.9 &                          2.9 &                  2.3 \\
MAXSAT-WPMS-2016       &                        3.9 &                 3.3 &                       3.3 &                               3.5 &                            7.2 &                 6.1 &                          3.7 &                  2.4 \\
MAXSAT12-PMS           &                        2.6 &                 2.6 &                       2.6 &                               2.6 &                            3.8 &                 4.9 &                          2.3 &                  2.8 \\
MAXSAT15-PMS-INDU      &                        1.8 &                 2.0 &                       2.0 &                               2.2 &                            6.8 &                 5.5 &                          2.3 &                  1.4 \\
MIP-2016               &                        3.2 &                 3.7 &                       2.7 &                               4.6 &                            4.1 &                 3.7 &                          3.2 &                  2.7 \\
PROTEUS-2014           &                       11.6 &                11.7 &                      11.8 &                              12.8 &                           24.0 &                18.4 &                         16.3 &                 13.5 \\
QBF-2011               &                        4.7 &                 4.6 &                       4.7 &                               5.3 &                            8.1 &                 8.1 &                          3.7 &                  5.3 \\
QBF-2014               &                        6.2 &                 5.9 &                       6.3 &                               7.5 &                           13.5 &                11.3 &                          7.4 &                  8.0 \\
QBF-2016               &                        7.0 &                 7.0 &                       7.0 &                               9.1 &                            9.8 &                 8.8 &                          8.9 &                  7.3 \\
SAT03-16\_INDU          &                        4.7 &                 4.7 &                       4.8 &                               5.8 &                            6.6 &                 6.4 &                          5.7 &                  8.4 \\
SAT11-HAND             &                       13.0 &                12.5 &                      11.6 &                              18.5 &                           18.3 &                22.6 &                         13.4 &                 20.9 \\
SAT11-INDU             &                       10.8 &                10.9 &                      11.2 &                               9.7 &                           11.7 &                15.0 &                         12.1 &                 12.2 \\
SAT11-RAND             &                        4.3 &                 3.7 &                       3.5 &                               4.3 &                            5.3 &                17.6 &                         10.5 &                  4.2 \\
SAT12-ALL              &                        8.5 &                 8.3 &                       8.3 &                               8.6 &                            8.3 &                15.9 &                          9.3 &                  9.2 \\
SAT12-HAND             &                       10.8 &                10.4 &                      10.4 &                              10.0 &                           12.7 &                19.9 &                          8.7 &                 12.7 \\
SAT12-INDU             &                        7.0 &                 7.1 &                       6.9 &                               7.6 &                            9.4 &                 9.7 &                          6.2 &                  7.9 \\
SAT12-RAND             &                        3.9 &                 3.5 &                       3.6 &                               4.0 &                           20.8 &                 4.5 &                          3.5 &                  4.3 \\
SAT15-INDU             &                        8.3 &                 8.3 &                       7.5 &                               6.6 &                            7.5 &                 6.9 &                          6.5 &                  8.3 \\
TSP-LION2015           &                        0.3 &                 0.3 &                       0.3 &                               0.2 &                            7.1 &                 2.6 &                          4.7 &                  1.2 \\
\midrule
 Mean &  5.7 & 5.6 & 5.6 & 6.1 & 9.1 & 9.5 & 6.4 & 6.6 \\
 Median &  4.5 & 4.2 &  4.2 & 4.9 & 7.8 & 8.4 & 6.0 & 4.8 \\
\bottomrule
\end{tabular}

==> figures/scatter_asf.tex <==
\begin{tikzpicture}
	\begin{axis}[%
	xmin=0,
	ymax=100,
	xmax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=AutoSurvivalForest,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.3619704970840113  0.678307188167013  ISAC*LIKE
0.1896392797062668  0.37057365073897225  ISAC*LIKE
0.4885481210537633  0.5816052568612295  ISAC*LIKE
0.2856889145572622  0.5228777822385304  ISAC*LIKE
2.574075453233949  25.005638168808908  ISAC*LIKE
0.3354411269837004  0.633979482712966  ISAC*LIKE
1.0116773331890154  0.7481160175040764  ISAC*LIKE
0.18842793802823307  0.3261541897619934  ISAC*LIKE
0.4133490247933328  0.6389066027778655  ISAC*LIKE
0.11745385536136335  0.5812831273846424  ISAC*LIKE
0.7405963051347608  0.9934845900321652  ISAC*LIKE
0.11066999294849617  0.3413740797208365  ISAC*LIKE
0.3668520683585846  0.7624399041017158  ISAC*LIKE
0.2690839315836035  0.4861309454590885  ISAC*LIKE
0.41599062484434457  1.00515320448719  ISAC*LIKE
0.9195871559690609  1.0863970459350147  ISAC*LIKE
0.6841207546775827  0.9530686135732818  ISAC*LIKE
0.9387152543158956  0.9781483425377416  ISAC*LIKE
0.4598447342846818  0.7013855838560397  ISAC*LIKE
8.19537516141494  3.0343187770427167  ISAC*LIKE
0.4660467725106746  0.6258720210231875  ISAC*LIKE
0.1975875599291004  0.8326084433409955  ISAC*LIKE
2.3536212972027872  4.635001851451788  ISAC*LIKE
0.5717033062529501  1.0160971015557598  ISAC*LIKE
0.7224238489198411  0.9580734424707004  ISAC*LIKE
0.30079348539086304  0.6527293218054211  ISAC*LIKE
0.3619704970840113  0.3727068040715841  PERALGORITHMREGRESSOR
0.1896392797062668  0.3561022296987444  PERALGORITHMREGRESSOR
0.4885481210537633  0.6127153109711706  PERALGORITHMREGRESSOR
0.2856889145572622  0.3549811173547622  PERALGORITHMREGRESSOR
2.574075453233949  2.390995304730814  PERALGORITHMREGRESSOR
0.3354411269837004  0.326774931576485  PERALGORITHMREGRESSOR
1.0116773331890154  0.7245332418766008  PERALGORITHMREGRESSOR
0.18842793802823307  0.2171794958650953  PERALGORITHMREGRESSOR
0.4133490247933328  0.4521638388413735  PERALGORITHMREGRESSOR
0.11745385536136335  0.1365715014720295  PERALGORITHMREGRESSOR
0.7405963051347608  0.7798023256886788  PERALGORITHMREGRESSOR
0.11066999294849617  0.125197658996884  PERALGORITHMREGRESSOR
0.3668520683585846  0.3900456945793733  PERALGORITHMREGRESSOR
0.2690839315836035  0.2565890812097911  PERALGORITHMREGRESSOR
0.41599062484434457  0.4220812771207481  PERALGORITHMREGRESSOR
0.9195871559690609  1.0369553794225423  PERALGORITHMREGRESSOR
0.6841207546775827  0.6089795737986103  PERALGORITHMREGRESSOR
0.9387152543158956  0.909550971459662  PERALGORITHMREGRESSOR
0.4598447342846818  0.5092849527012576  PERALGORITHMREGRESSOR
8.19537516141494  10.046493826664182  PERALGORITHMREGRESSOR
0.4660467725106746  0.6703583113478012  PERALGORITHMREGRESSOR
0.1975875599291004  0.17656354601663074  PERALGORITHMREGRESSOR
2.3536212972027872  4.018239865130491  PERALGORITHMREGRESSOR
0.5717033062529501  0.6461771054988412  PERALGORITHMREGRESSOR
0.7224238489198411  0.868896361056391  PERALGORITHMREGRESSOR
0.30079348539086304  0.3173743198219577  PERALGORITHMREGRESSOR
0.3619704970840113  0.4157567289098781  SUNNY*LIKE
0.1896392797062668  0.3420544115873054  SUNNY*LIKE
0.4885481210537633  0.5102692334591704  SUNNY*LIKE
0.2856889145572622  0.38778415792083704  SUNNY*LIKE
2.574075453233949  11.024140970070023  SUNNY*LIKE
0.3354411269837004  0.4199871970968848  SUNNY*LIKE
1.0116773331890154  1.0144015263116142  SUNNY*LIKE
0.18842793802823307  0.2342363871867101  SUNNY*LIKE
0.4133490247933328  0.472568787142205  SUNNY*LIKE
0.11745385536136335  0.13413782935635393  SUNNY*LIKE
0.7405963051347608  0.8264661375466948  SUNNY*LIKE
0.11066999294849617  0.13519036320762598  SUNNY*LIKE
0.3668520683585846  0.28487456563991603  SUNNY*LIKE
0.2690839315836035  0.27891490037641364  SUNNY*LIKE
0.41599062484434457  0.24347647329399344  SUNNY*LIKE
0.9195871559690609  1.1005666866952357  SUNNY*LIKE
0.6841207546775827  0.7690655151737142  SUNNY*LIKE
0.9387152543158956  0.9877233823201352  SUNNY*LIKE
0.4598447342846818  0.5190616864954294  SUNNY*LIKE
8.19537516141494  8.895331064742077  SUNNY*LIKE
0.4660467725106746  0.5613114268682801  SUNNY*LIKE
0.1975875599291004  0.24146530135189825  SUNNY*LIKE
2.3536212972027872  11.525693770202654  SUNNY*LIKE
0.5717033062529501  0.4872517183107655  SUNNY*LIKE
0.7224238489198411  0.8194358754277964  SUNNY*LIKE
0.30079348539086304  0.19807847047517213  SUNNY*LIKE
0.3619704970840113  0.4025668486665903  SATZILLA'11*LIKE
0.1896392797062668  0.29502449425618205  SATZILLA'11*LIKE
0.4885481210537633  0.6201886117590589  SATZILLA'11*LIKE
0.2856889145572622  0.34692854380740423  SATZILLA'11*LIKE
2.574075453233949  40.47124191666446  SATZILLA'11*LIKE
0.3354411269837004  0.2821401701836627  SATZILLA'11*LIKE
1.0116773331890154  0.7281512246422769  SATZILLA'11*LIKE
0.18842793802823307  0.15409546878934588  SATZILLA'11*LIKE
0.4133490247933328  0.56949283393721  SATZILLA'11*LIKE
0.11745385536136335  0.36224385773615614  SATZILLA'11*LIKE
0.7405963051347608  0.6409090386556566  SATZILLA'11*LIKE
0.11066999294849617  0.2072072017576949  SATZILLA'11*LIKE
0.3668520683585846  0.4662401081022946  SATZILLA'11*LIKE
0.2690839315836035  0.2383579026242359  SATZILLA'11*LIKE
0.41599062484434457  0.4013072777852713  SATZILLA'11*LIKE
0.9195871559690609  0.8918135633190942  SATZILLA'11*LIKE
0.6841207546775827  0.7909236746193591  SATZILLA'11*LIKE
0.9387152543158956  0.8511395055215155  SATZILLA'11*LIKE
0.4598447342846818  0.40416828060962395  SATZILLA'11*LIKE
8.19537516141494  9.040038521329254  SATZILLA'11*LIKE
0.4660467725106746  0.4382131452252581  SATZILLA'11*LIKE
0.1975875599291004  0.17632633083365565  SATZILLA'11*LIKE
2.3536212972027872  4.728210093497262  SATZILLA'11*LIKE
0.5717033062529501  0.5884760955910446  SATZILLA'11*LIKE
0.7224238489198411  0.8541750308083232  SATZILLA'11*LIKE
0.30079348539086304  0.4688268909116234  SATZILLA'11*LIKE
0.3619704970840113  0.3661192613385954  MULTICLASSSELECTOR
0.1896392797062668  0.7816601153543972  MULTICLASSSELECTOR
0.4885481210537633  0.6765204702029799  MULTICLASSSELECTOR
0.2856889145572622  0.6292123480351777  MULTICLASSSELECTOR
2.574075453233949  59.70167589543316  MULTICLASSSELECTOR
0.3354411269837004  0.4125744853023916  MULTICLASSSELECTOR
1.0116773331890154  0.8613737468472333  MULTICLASSSELECTOR
0.18842793802823307  0.3333403316545537  MULTICLASSSELECTOR
0.4133490247933328  0.8372401386776829  MULTICLASSSELECTOR
0.11745385536136335  0.17342325582160995  MULTICLASSSELECTOR
0.7405963051347608  0.9426330676164544  MULTICLASSSELECTOR
0.11066999294849617  0.31028969535327755  MULTICLASSSELECTOR
0.3668520683585846  0.841125297437588  MULTICLASSSELECTOR
0.2690839315836035  0.3707292833375948  MULTICLASSSELECTOR
0.41599062484434457  1.2440671401636696  MULTICLASSSELECTOR
0.9195871559690609  5.316655519540719  MULTICLASSSELECTOR
0.6841207546775827  0.75823175512707  MULTICLASSSELECTOR
0.9387152543158956  0.9358700154462076  MULTICLASSSELECTOR
0.4598447342846818  0.6089544785846619  MULTICLASSSELECTOR
8.19537516141494  9.745508035939428  MULTICLASSSELECTOR
0.4660467725106746  0.5741456751186104  MULTICLASSSELECTOR
0.1975875599291004  0.31481281763565755  MULTICLASSSELECTOR
2.3536212972027872  8.762749094703938  MULTICLASSSELECTOR
0.5717033062529501  1.1773932311669637  MULTICLASSSELECTOR
0.7224238489198411  0.9938409073890452  MULTICLASSSELECTOR
0.30079348539086304  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
	    (0.2,0.2)
	    (0.3,0.3)
	    (0.4,0.4)
	    (0.5,0.5)
	    (0.6,0.6)
	    (0.7,0.7)
	    (0.8,0.8)
	    (0.9,0.9)
	    (1,1)
	    (1.5,1.5)
		(2,2)
		(3,3)
		(4,4)
		(5,5)
		(6,6)
		(7,7)
		(8,8)
		(10,10)
		(100,100)
	};
	\end{axis}
\end{tikzpicture}

==> figures/scatter_esf.tex <==
\begin{tikzpicture}
	\begin{semilogyaxis}[%
	xmin=0,
	xmax=100,
	ymax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=ExpectationSurvivalForest,
	log ticks with fixed point,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.36631947541879695  0.678307188167013  ISAC*LIKE
0.2592832599339565  0.37057365073897225  ISAC*LIKE
0.4744089449595796  0.5816052568612295  ISAC*LIKE
0.3007385914842758  0.5228777822385304  ISAC*LIKE
2.5766243051276114  25.005638168808908  ISAC*LIKE
0.34902915573329063  0.633979482712966  ISAC*LIKE
1.0106928871325442  0.7481160175040764  ISAC*LIKE
0.1934212219443083  0.3261541897619934  ISAC*LIKE
0.4083934578602521  0.6389066027778655  ISAC*LIKE
0.13551202514865812  0.5812831273846424  ISAC*LIKE
0.7322069990826827  0.9934845900321652  ISAC*LIKE
0.11120358643431127  0.3413740797208365  ISAC*LIKE
0.4596011123631822  0.7624399041017158  ISAC*LIKE
0.2690613866762786  0.4861309454590885  ISAC*LIKE
0.3891742445877905  1.00515320448719  ISAC*LIKE
0.9953247242720892  1.0863970459350147  ISAC*LIKE
0.6573188045299808  0.9530686135732818  ISAC*LIKE
0.9733953124318652  0.9781483425377416  ISAC*LIKE
0.4603411780387689  0.7013855838560397  ISAC*LIKE
4.531596581362732  3.0343187770427167  ISAC*LIKE
0.5147341205889762  0.6258720210231875  ISAC*LIKE
0.20438456695669927  0.8326084433409955  ISAC*LIKE
2.400257262697644  4.635001851451788  ISAC*LIKE
0.5696449903581586  1.0160971015557598  ISAC*LIKE
0.7227773541996839  0.9580734424707004  ISAC*LIKE
0.3007482452133336  0.6527293218054211  ISAC*LIKE
0.36631947541879695  0.3727068040715841  PERALGORITHMREGRESSOR
0.2592832599339565  0.3561022296987444  PERALGORITHMREGRESSOR
0.4744089449595796  0.6127153109711706  PERALGORITHMREGRESSOR
0.3007385914842758  0.3549811173547622  PERALGORITHMREGRESSOR
2.5766243051276114  2.390995304730814  PERALGORITHMREGRESSOR
0.34902915573329063  0.326774931576485  PERALGORITHMREGRESSOR
1.0106928871325442  0.7245332418766008  PERALGORITHMREGRESSOR
0.1934212219443083  0.2171794958650953  PERALGORITHMREGRESSOR
0.4083934578602521  0.4521638388413735  PERALGORITHMREGRESSOR
0.13551202514865812  0.1365715014720295  PERALGORITHMREGRESSOR
0.7322069990826827  0.7798023256886788  PERALGORITHMREGRESSOR
0.11120358643431127  0.125197658996884  PERALGORITHMREGRESSOR
0.4596011123631822  0.3900456945793733  PERALGORITHMREGRESSOR
0.2690613866762786  0.2565890812097911  PERALGORITHMREGRESSOR
0.3891742445877905  0.4220812771207481  PERALGORITHMREGRESSOR
0.9953247242720892  1.0369553794225423  PERALGORITHMREGRESSOR
0.6573188045299808  0.6089795737986103  PERALGORITHMREGRESSOR
0.9733953124318652  0.909550971459662  PERALGORITHMREGRESSOR
0.4603411780387689  0.5092849527012576  PERALGORITHMREGRESSOR
4.531596581362732  10.046493826664182  PERALGORITHMREGRESSOR
0.5147341205889762  0.6703583113478012  PERALGORITHMREGRESSOR
0.20438456695669927  0.17656354601663074  PERALGORITHMREGRESSOR
2.400257262697644  4.018239865130491  PERALGORITHMREGRESSOR
0.5696449903581586  0.6461771054988412  PERALGORITHMREGRESSOR
0.7227773541996839  0.868896361056391  PERALGORITHMREGRESSOR
0.3007482452133336  0.3173743198219577  PERALGORITHMREGRESSOR
0.36631947541879695  0.4157567289098781  SUNNY*LIKE
0.2592832599339565  0.3420544115873054  SUNNY*LIKE
0.4744089449595796  0.5102692334591704  SUNNY*LIKE
0.3007385914842758  0.38778415792083704  SUNNY*LIKE
2.5766243051276114  11.024140970070023  SUNNY*LIKE
0.34902915573329063  0.4199871970968848  SUNNY*LIKE
1.0106928871325442  1.0144015263116142  SUNNY*LIKE
0.1934212219443083  0.2342363871867101  SUNNY*LIKE
0.4083934578602521  0.472568787142205  SUNNY*LIKE
0.13551202514865812  0.13413782935635393  SUNNY*LIKE
0.7322069990826827  0.8264661375466948  SUNNY*LIKE
0.11120358643431127  0.13519036320762598  SUNNY*LIKE
0.4596011123631822  0.28487456563991603  SUNNY*LIKE
0.2690613866762786  0.27891490037641364  SUNNY*LIKE
0.3891742445877905  0.24347647329399344  SUNNY*LIKE
0.9953247242720892  1.1005666866952357  SUNNY*LIKE
0.6573188045299808  0.7690655151737142  SUNNY*LIKE
0.9733953124318652  0.9877233823201352  SUNNY*LIKE
0.4603411780387689  0.5190616864954294  SUNNY*LIKE
4.531596581362732  8.895331064742077  SUNNY*LIKE
0.5147341205889762  0.5613114268682801  SUNNY*LIKE
0.20438456695669927  0.24146530135189825  SUNNY*LIKE
2.400257262697644  11.525693770202654  SUNNY*LIKE
0.5696449903581586  0.4872517183107655  SUNNY*LIKE
0.7227773541996839  0.8194358754277964  SUNNY*LIKE
0.3007482452133336  0.19807847047517213  SUNNY*LIKE
0.36631947541879695  0.4025668486665903  SATZILLA'11*LIKE
0.2592832599339565  0.29502449425618205  SATZILLA'11*LIKE
0.4744089449595796  0.6201886117590589  SATZILLA'11*LIKE
0.3007385914842758  0.34692854380740423  SATZILLA'11*LIKE
2.5766243051276114  40.47124191666446  SATZILLA'11*LIKE
0.34902915573329063  0.2821401701836627  SATZILLA'11*LIKE
1.0106928871325442  0.7281512246422769  SATZILLA'11*LIKE
0.1934212219443083  0.15409546878934588  SATZILLA'11*LIKE
0.4083934578602521  0.56949283393721  SATZILLA'11*LIKE
0.13551202514865812  0.36224385773615614  SATZILLA'11*LIKE
0.7322069990826827  0.6409090386556566  SATZILLA'11*LIKE
0.11120358643431127  0.2072072017576949  SATZILLA'11*LIKE
0.4596011123631822  0.4662401081022946  SATZILLA'11*LIKE
0.2690613866762786  0.2383579026242359  SATZILLA'11*LIKE
0.3891742445877905  0.4013072777852713  SATZILLA'11*LIKE
0.9953247242720892  0.8918135633190942  SATZILLA'11*LIKE
0.6573188045299808  0.7909236746193591  SATZILLA'11*LIKE
0.9733953124318652  0.8511395055215155  SATZILLA'11*LIKE
0.4603411780387689  0.40416828060962395  SATZILLA'11*LIKE
4.531596581362732  9.040038521329254  SATZILLA'11*LIKE
0.5147341205889762  0.4382131452252581  SATZILLA'11*LIKE
0.20438456695669927  0.17632633083365565  SATZILLA'11*LIKE
2.400257262697644  4.728210093497262  SATZILLA'11*LIKE
0.5696449903581586  0.5884760955910446  SATZILLA'11*LIKE
0.7227773541996839  0.8541750308083232  SATZILLA'11*LIKE
0.3007482452133336  0.4688268909116234  SATZILLA'11*LIKE
0.36631947541879695  0.3661192613385954  MULTICLASSSELECTOR
0.2592832599339565  0.7816601153543972  MULTICLASSSELECTOR
0.4744089449595796  0.6765204702029799  MULTICLASSSELECTOR
0.3007385914842758  0.6292123480351777  MULTICLASSSELECTOR
2.5766243051276114  59.70167589543316  MULTICLASSSELECTOR
0.34902915573329063  0.4125744853023916  MULTICLASSSELECTOR
1.0106928871325442  0.8613737468472333  MULTICLASSSELECTOR
0.1934212219443083  0.3333403316545537  MULTICLASSSELECTOR
0.4083934578602521  0.8372401386776829  MULTICLASSSELECTOR
0.13551202514865812  0.17342325582160995  MULTICLASSSELECTOR
0.7322069990826827  0.9426330676164544  MULTICLASSSELECTOR
0.11120358643431127  0.31028969535327755  MULTICLASSSELECTOR
0.4596011123631822  0.841125297437588  MULTICLASSSELECTOR
0.2690613866762786  0.3707292833375948  MULTICLASSSELECTOR
0.3891742445877905  1.2440671401636696  MULTICLASSSELECTOR
0.9953247242720892  5.316655519540719  MULTICLASSSELECTOR
0.6573188045299808  0.75823175512707  MULTICLASSSELECTOR
0.9733953124318652  0.9358700154462076  MULTICLASSSELECTOR
0.4603411780387689  0.6089544785846619  MULTICLASSSELECTOR
4.531596581362732  9.745508035939428  MULTICLASSSELECTOR
0.5147341205889762  0.5741456751186104  MULTICLASSSELECTOR
0.20438456695669927  0.31481281763565755  MULTICLASSSELECTOR
2.400257262697644  8.762749094703938  MULTICLASSSELECTOR
0.5696449903581586  1.1773932311669637  MULTICLASSSELECTOR
0.7227773541996839  0.9938409073890452  MULTICLASSSELECTOR
0.3007482452133336  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
		(100,100)
	};
	\end{semilogyaxis}
\end{tikzpicture}

==> figures/scatter_gssf.tex <==
\begin{tikzpicture}
	\begin{semilogyaxis}[%
	xmin=0,
	xmax=100,
	ymax=100,
	ymin=0,
	xmode=log,
	ymode=log,
	legend pos=outer north east,
    tick style={grid=major},
	xlabel=nPAR10 GridSearchSurvivalForest,
	ylabel=nPAR10 Baseline,
	log ticks with fixed point,
	scatter/classes={%
	    MULTICLASSSELECTOR={mark=square,brown},%
		PERALGORITHMREGRESSOR={mark=square,red},%
		ISAC*LIKE={mark=o,blue},
		SATZILLA'11*LIKE={mark=o,black},%
		SUNNY*LIKE={mark=o,magenta}}]
	\addplot[scatter,only marks,%
		scatter src=explicit symbolic]%
	table[meta=label] {
x     y      label
0.3595703063406438  0.678307188167013  ISAC*LIKE
0.24237898483093134  0.37057365073897225  ISAC*LIKE
0.4885539473876691  0.5816052568612295  ISAC*LIKE
0.3037088355194861  0.5228777822385304  ISAC*LIKE
2.577448890275856  25.005638168808908  ISAC*LIKE
0.3355424548592121  0.633979482712966  ISAC*LIKE
0.94590081392888  0.7481160175040764  ISAC*LIKE
0.19233936774392985  0.3261541897619934  ISAC*LIKE
0.4156346977057006  0.6389066027778655  ISAC*LIKE
0.11009614002362557  0.5812831273846424  ISAC*LIKE
0.7268223371245681  0.9934845900321652  ISAC*LIKE
0.11390021428666255  0.3413740797208365  ISAC*LIKE
0.36938359885355504  0.7624399041017158  ISAC*LIKE
0.2691410807256949  0.4861309454590885  ISAC*LIKE
0.414190330188758  1.00515320448719  ISAC*LIKE
0.9561134869872088  1.0863970459350147  ISAC*LIKE
0.7036296835341059  0.9530686135732818  ISAC*LIKE
0.8960219654197135  0.9781483425377416  ISAC*LIKE
0.5603193890982832  0.7013855838560397  ISAC*LIKE
4.393978741958076  3.0343187770427167  ISAC*LIKE
0.3854524480930018  0.6258720210231875  ISAC*LIKE
0.20539526376817102  0.8326084433409955  ISAC*LIKE
2.3858604230905835  4.635001851451788  ISAC*LIKE
0.5761557175705883  1.0160971015557598  ISAC*LIKE
0.7399812539598516  0.9580734424707004  ISAC*LIKE
0.3363421530290565  0.6527293218054211  ISAC*LIKE
0.3595703063406438  0.3727068040715841  PERALGORITHMREGRESSOR
0.24237898483093134  0.3561022296987444  PERALGORITHMREGRESSOR
0.4885539473876691  0.6127153109711706  PERALGORITHMREGRESSOR
0.3037088355194861  0.3549811173547622  PERALGORITHMREGRESSOR
2.577448890275856  2.390995304730814  PERALGORITHMREGRESSOR
0.3355424548592121  0.326774931576485  PERALGORITHMREGRESSOR
0.94590081392888  0.7245332418766008  PERALGORITHMREGRESSOR
0.19233936774392985  0.2171794958650953  PERALGORITHMREGRESSOR
0.4156346977057006  0.4521638388413735  PERALGORITHMREGRESSOR
0.11009614002362557  0.1365715014720295  PERALGORITHMREGRESSOR
0.7268223371245681  0.7798023256886788  PERALGORITHMREGRESSOR
0.11390021428666255  0.125197658996884  PERALGORITHMREGRESSOR
0.36938359885355504  0.3900456945793733  PERALGORITHMREGRESSOR
0.2691410807256949  0.2565890812097911  PERALGORITHMREGRESSOR
0.414190330188758  0.4220812771207481  PERALGORITHMREGRESSOR
0.9561134869872088  1.0369553794225423  PERALGORITHMREGRESSOR
0.7036296835341059  0.6089795737986103  PERALGORITHMREGRESSOR
0.8960219654197135  0.909550971459662  PERALGORITHMREGRESSOR
0.5603193890982832  0.5092849527012576  PERALGORITHMREGRESSOR
4.393978741958076  10.046493826664182  PERALGORITHMREGRESSOR
0.3854524480930018  0.6703583113478012  PERALGORITHMREGRESSOR
0.20539526376817102  0.17656354601663074  PERALGORITHMREGRESSOR
2.3858604230905835  4.018239865130491  PERALGORITHMREGRESSOR
0.5761557175705883  0.6461771054988412  PERALGORITHMREGRESSOR
0.7399812539598516  0.868896361056391  PERALGORITHMREGRESSOR
0.3363421530290565  0.3173743198219577  PERALGORITHMREGRESSOR
0.3595703063406438  0.4157567289098781  SUNNY*LIKE
0.24237898483093134  0.3420544115873054  SUNNY*LIKE
0.4885539473876691  0.5102692334591704  SUNNY*LIKE
0.3037088355194861  0.38778415792083704  SUNNY*LIKE
2.577448890275856  11.024140970070023  SUNNY*LIKE
0.3355424548592121  0.4199871970968848  SUNNY*LIKE
0.94590081392888  1.0144015263116142  SUNNY*LIKE
0.19233936774392985  0.2342363871867101  SUNNY*LIKE
0.4156346977057006  0.472568787142205  SUNNY*LIKE
0.11009614002362557  0.13413782935635393  SUNNY*LIKE
0.7268223371245681  0.8264661375466948  SUNNY*LIKE
0.11390021428666255  0.13519036320762598  SUNNY*LIKE
0.36938359885355504  0.28487456563991603  SUNNY*LIKE
0.2691410807256949  0.27891490037641364  SUNNY*LIKE
0.414190330188758  0.24347647329399344  SUNNY*LIKE
0.9561134869872088  1.1005666866952357  SUNNY*LIKE
0.7036296835341059  0.7690655151737142  SUNNY*LIKE
0.8960219654197135  0.9877233823201352  SUNNY*LIKE
0.5603193890982832  0.5190616864954294  SUNNY*LIKE
4.393978741958076  8.895331064742077  SUNNY*LIKE
0.3854524480930018  0.5613114268682801  SUNNY*LIKE
0.20539526376817102  0.24146530135189825  SUNNY*LIKE
2.3858604230905835  11.525693770202654  SUNNY*LIKE
0.5761557175705883  0.4872517183107655  SUNNY*LIKE
0.7399812539598516  0.8194358754277964  SUNNY*LIKE
0.3363421530290565  0.19807847047517213  SUNNY*LIKE
0.3595703063406438  0.4025668486665903  SATZILLA'11*LIKE
0.24237898483093134  0.29502449425618205  SATZILLA'11*LIKE
0.4885539473876691  0.6201886117590589  SATZILLA'11*LIKE
0.3037088355194861  0.34692854380740423  SATZILLA'11*LIKE
2.577448890275856  40.47124191666446  SATZILLA'11*LIKE
0.3355424548592121  0.2821401701836627  SATZILLA'11*LIKE
0.94590081392888  0.7281512246422769  SATZILLA'11*LIKE
0.19233936774392985  0.15409546878934588  SATZILLA'11*LIKE
0.4156346977057006  0.56949283393721  SATZILLA'11*LIKE
0.11009614002362557  0.36224385773615614  SATZILLA'11*LIKE
0.7268223371245681  0.6409090386556566  SATZILLA'11*LIKE
0.11390021428666255  0.2072072017576949  SATZILLA'11*LIKE
0.36938359885355504  0.4662401081022946  SATZILLA'11*LIKE
0.2691410807256949  0.2383579026242359  SATZILLA'11*LIKE
0.414190330188758  0.4013072777852713  SATZILLA'11*LIKE
0.9561134869872088  0.8918135633190942  SATZILLA'11*LIKE
0.7036296835341059  0.7909236746193591  SATZILLA'11*LIKE
0.8960219654197135  0.8511395055215155  SATZILLA'11*LIKE
0.5603193890982832  0.40416828060962395  SATZILLA'11*LIKE
4.393978741958076  9.040038521329254  SATZILLA'11*LIKE
0.3854524480930018  0.4382131452252581  SATZILLA'11*LIKE
0.20539526376817102  0.17632633083365565  SATZILLA'11*LIKE
2.3858604230905835  4.728210093497262  SATZILLA'11*LIKE
0.5761557175705883  0.5884760955910446  SATZILLA'11*LIKE
0.7399812539598516  0.8541750308083232  SATZILLA'11*LIKE
0.3363421530290565  0.4688268909116234  SATZILLA'11*LIKE
0.3595703063406438  0.3661192613385954  MULTICLASSSELECTOR
0.24237898483093134  0.7816601153543972  MULTICLASSSELECTOR
0.4885539473876691  0.6765204702029799  MULTICLASSSELECTOR
0.3037088355194861  0.6292123480351777  MULTICLASSSELECTOR
2.577448890275856  59.70167589543316  MULTICLASSSELECTOR
0.3355424548592121  0.4125744853023916  MULTICLASSSELECTOR
0.94590081392888  0.8613737468472333  MULTICLASSSELECTOR
0.19233936774392985  0.3333403316545537  MULTICLASSSELECTOR
0.4156346977057006  0.8372401386776829  MULTICLASSSELECTOR
0.11009614002362557  0.17342325582160995  MULTICLASSSELECTOR
0.7268223371245681  0.9426330676164544  MULTICLASSSELECTOR
0.11390021428666255  0.31028969535327755  MULTICLASSSELECTOR
0.36938359885355504  0.841125297437588  MULTICLASSSELECTOR
0.2691410807256949  0.3707292833375948  MULTICLASSSELECTOR
0.414190330188758  1.2440671401636696  MULTICLASSSELECTOR
0.9561134869872088  5.316655519540719  MULTICLASSSELECTOR
0.7036296835341059  0.75823175512707  MULTICLASSSELECTOR
0.8960219654197135  0.9358700154462076  MULTICLASSSELECTOR
0.5603193890982832  0.6089544785846619  MULTICLASSSELECTOR
4.393978741958076  9.745508035939428  MULTICLASSSELECTOR
0.3854524480930018  0.5741456751186104  MULTICLASSSELECTOR
0.20539526376817102  0.31481281763565755  MULTICLASSSELECTOR
2.3858604230905835  8.762749094703938  MULTICLASSSELECTOR
0.5761557175705883  1.1773932311669637  MULTICLASSSELECTOR
0.7399812539598516  0.9938409073890452  MULTICLASSSELECTOR
0.3363421530290565  0.6669929035288492  MULTICLASSSELECTOR
%
};
	\addlegendentry{MultiClassSelector}
	\addlegendentry{PerAlgorithmRegressor}
	\addlegendentry{ISAC*LIKE}
	\addlegendentry{SATZILLA'11*LIKE}
	\addlegendentry{SUNNY*LIKE}
	\addplot[color=black,mark=None] coordinates {
	    (0.1,0.1)
		(100,100)
	};
	\end{semilogyaxis}
\end{tikzpicture}

==> tables/normalized_table.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
& \parbox{2.3cm}{\centering Auto-\\ SurvivalForest} & \parbox{2.3cm}{\centering Expectation-\\ SurvivalForest} & \parbox{2.3cm}{\centering GridSearch-\\ SurvivalForest} &  \parbox{1.7cm}{\centering ISAC\\ *like} &  \parbox{2.0cm}{\centering MultiClass-\\ Selector} & \parbox{2.5cm}{\centering PerAlgorithm-\\ Regressor} &  \parbox{2.2cm}{\centering SATzilla'11\\ *like} &  \parbox{1.7cm}{\centering SUNNY\\ *like} \\
ASlib Scenario         &                     &                            &                           &            &                     &                        &                   &             \\
\midrule
ASP-POTASSCO           &            0.300793 &                   0.300748 &                  0.336342 &   0.652729 &            0.666993 &               0.320221 &          0.428925 &    0.172295 \\
BNSL-2016              &            0.197588 &                   0.204385 &                  0.205395 &   0.832608 &            0.314813 &               0.203520 &          0.197481 &    0.248938 \\
CPMP-2015              &            0.938715 &                   0.973395 &                  0.896022 &   0.978148 &            0.935870 &               0.882819 &          0.848480 &    1.050350 \\
CSP-2010               &            0.189639 &                   0.259283 &                  0.242379 &   0.370574 &            0.781660 &               0.365766 &          0.241954 &    0.402470 \\
CSP-MZN-2013           &            0.110670 &                   0.111204 &                  0.113900 &   0.341374 &            0.310290 &               0.135796 &          0.209275 &    0.125618 \\
CSP-Minizinc-Time-2016 &            0.459845 &                   0.460341 &                  0.560319 &   0.701386 &            0.608954 &               0.512432 &          0.502317 &    0.519079 \\
GRAPHS-2015            &            2.353621 &                   2.400257 &                  2.385860 &   4.635002 &            8.762749 &               5.960256 &          8.226409 &   11.525636 \\
MAXSAT-PMS-2016        &            0.571703 &                   0.569645 &                  0.576156 &   1.016097 &            1.177393 &               0.746590 &          0.591542 &    0.487082 \\
MAXSAT-WPMS-2016       &            0.366852 &                   0.459601 &                  0.369384 &   0.762440 &            0.841125 &               0.471578 &          0.429294 &    0.244580 \\
MAXSAT12-PMS           &            0.269084 &                   0.269061 &                  0.269141 &   0.486131 &            0.370729 &               0.302595 &          0.240272 &    0.278908 \\
MAXSAT15-PMS-INDU      &            0.415991 &                   0.389174 &                  0.414190 &   1.005153 &            1.244067 &               0.535373 &          0.430227 &    0.243505 \\
MIP-2016               &            8.195375 &                   4.531597 &                  4.393979 &   3.034319 &            9.745508 &              10.143470 &          9.662852 &    8.855730 \\
PROTEUS-2014           &            0.413349 &                   0.408393 &                  0.415635 &   0.638907 &            0.837240 &               0.450890 &          0.576535 &    0.473812 \\
QBF-2011               &            0.188428 &                   0.193421 &                  0.192339 &   0.326154 &            0.333340 &               0.195713 &          0.165905 &    0.220605 \\
QBF-2014               &            0.285689 &                   0.300739 &                  0.303709 &   0.522878 &            0.629212 &               0.334371 &          0.359988 &    0.397089 \\
QBF-2016               &            0.488548 &                   0.474409 &                  0.488554 &   0.581605 &            0.676520 &               0.626964 &          0.643596 &    0.510265 \\
SAT03-16\_INDU          &            0.722424 &                   0.722777 &                  0.739981 &   0.958073 &            0.993841 &               0.845725 &          0.882314 &    0.845817 \\
SAT11-HAND             &            0.466047 &                   0.514734 &                  0.385452 &   0.625872 &            0.574146 &               0.453943 &          0.453614 &    0.697061 \\
SAT11-INDU             &            0.684121 &                   0.657319 &                  0.703630 &   0.953069 &            0.758232 &               0.624086 &          0.842440 &    0.848683 \\
SAT11-RAND             &            0.117454 &                   0.135512 &                  0.110096 &   0.581283 &            0.173423 &               0.114355 &          0.374920 &    0.133021 \\
SAT12-ALL              &            0.361970 &                   0.366319 &                  0.359570 &   0.678307 &            0.366119 &               0.361825 &          0.428101 &    0.396569 \\
SAT12-HAND             &            0.335441 &                   0.349029 &                  0.335542 &   0.633979 &            0.412574 &               0.360927 &          0.305365 &    0.415547 \\
SAT12-INDU             &            0.740596 &                   0.732207 &                  0.726822 &   0.993485 &            0.942633 &               0.817029 &          0.642115 &    0.812497 \\
SAT12-RAND             &            0.919587 &                   0.995325 &                  0.956113 &   1.086397 &            5.316656 &               1.242140 &          0.916708 &    1.108742 \\
SAT15-INDU             &            1.011677 &                   1.010693 &                  0.945901 &   0.748116 &            0.861374 &               0.968517 &          0.804147 &    1.035853 \\
TSP-LION2015           &            2.574075 &                   2.576624 &                  2.577449 &  25.005638 &           59.701676 &               2.155110 &         41.317910 &   11.024178 \\
\bottomrule
\end{tabular}

==> tables/unsolved_table.tex <==
\begin{tabular}{l||rrr|rrrrr}
\toprule

 &  \parbox{2.3cm}{\centering Expectation-\\ SurvivalForest\\} &  \parbox{2.3cm}{\centering Auto-\\ SurvivalForest\\} &  \parbox{2.3cm}{\centering GridSearch-\\ SurvivalForest\\} &  \parbox{2.8cm}{\centering PerAlgorithm-\\Regressor\\(Runtime)} &  \parbox{2.0cm}{\centering MultiClass-\\Selector\\(Runtime)} &  \parbox{1.7cm}{\centering ISAC\\ *like\\(PAR10)} & \parbox{2.2cm}{\centering SATzilla'11\\ *like\\(Runtime)}  &  \parbox{1.7cm}{\centering SUNNY\\ *like\\(PAR10)} \\

\midrule
ASP-POTASSCO           &                        2.2 &                 2.2 &                       2.5 &                               2.4 &                            5.5 &                 5.3 &                          3.7 &                  1.3 \\
BNSL-2016              &                        2.4 &                 2.3 &                       2.4 &                               2.0 &                            3.8 &                10.0 &                          2.2 &                  3.0 \\
CPMP-2015              &                       15.8 &                15.2 &                      14.4 &                              14.4 &                           15.4 &                16.7 &                         14.0 &                 18.2 \\
CSP-2010               &                        0.6 &                 0.4 &                       0.5 &                               0.7 &                            1.5 &                 0.9 &                          0.6 &                  0.8 \\
CSP-MZN-2013           &                        3.5 &                 3.5 &                       3.6 &                               4.0 &                           10.6 &                11.6 &                          7.0 &                  4.0 \\
CSP-Minizinc-Time-2016 &                        8.7 &                 8.7 &                       9.9 &                               8.4 &                            8.4 &                 9.8 &                          7.4 &                  8.8 \\
GRAPHS-2015            &                        0.5 &                 0.5 &                       0.5 &                               0.6 &                            1.1 &                 0.7 &                          0.8 &                  0.5 \\
MAXSAT-PMS-2016        &                        2.5 &                 2.5 &                       2.5 &                               3.2 &                            5.6 &                 4.9 &                          2.9 &                  2.3 \\
MAXSAT-WPMS-2016       &                        3.9 &                 3.3 &                       3.3 &                               3.5 &                            7.2 &                 6.1 &                          3.7 &                  2.4 \\
MAXSAT12-PMS           &                        2.6 &                 2.6 &                       2.6 &                               2.6 &                            3.8 &                 4.9 &                          2.3 &                  2.8 \\
MAXSAT15-PMS-INDU      &                        1.8 &                 2.0 &                       2.0 &                               2.2 &                            6.8 &                 5.5 &                          2.3 &                  1.4 \\
MIP-2016               &                        3.2 &                 3.7 &                       2.7 &                               4.6 &                            4.1 &                 3.7 &                          3.2 &                  2.7 \\
PROTEUS-2014           &                       11.6 &                11.7 &                      11.8 &                              12.8 &                           24.0 &                18.4 &                         16.3 &                 13.5 \\
QBF-2011               &                        4.7 &                 4.6 &                       4.7 &                               5.3 &                            8.1 &                 8.1 &                          3.7 &                  5.3 \\
QBF-2014               &                        6.2 &                 5.9 &                       6.3 &                               7.5 &                           13.5 &                11.3 &                          7.4 &                  8.0 \\
QBF-2016               &                        7.0 &                 7.0 &                       7.0 &                               9.1 &                            9.8 &                 8.8 &                          8.9 &                  7.3 \\
SAT03-16\_INDU          &                        4.7 &                 4.7 &                       4.8 &                               5.8 &                            6.6 &                 6.4 &                          5.7 &                  8.4 \\
SAT11-HAND             &                       13.0 &                12.5 &                      11.6 &                              18.5 &                           18.3 &                22.6 &                         13.4 &                 20.9 \\
SAT11-INDU             &                       10.8 &                10.9 &                      11.2 &                               9.7 &                           11.7 &                15.0 &                         12.1 &                 12.2 \\
SAT11-RAND             &                        4.3 &                 3.7 &                       3.5 &                               4.3 &                            5.3 &                17.6 &                         10.5 &                  4.2 \\
SAT12-ALL              &                        8.5 &                 8.3 &                       8.3 &                               8.6 &                            8.3 &                15.9 &                          9.3 &                  9.2 \\
SAT12-HAND             &                       10.8 &                10.4 &                      10.4 &                              10.0 &                           12.7 &                19.9 &                          8.7 &                 12.7 \\
SAT12-INDU             &                        7.0 &                 7.1 &                       6.9 &                               7.6 &                            9.4 &                 9.7 &                          6.2 &                  7.9 \\
SAT12-RAND             &                        3.9 &                 3.5 &                       3.6 &                               4.0 &                           20.8 &                 4.5 &                          3.5 &                  4.3 \\
SAT15-INDU             &                        8.3 &                 8.3 &                       7.5 &                               6.6 &                            7.5 &                 6.9 &                          6.5 &                  8.3 \\
TSP-LION2015           &                        0.3 &                 0.3 &                       0.3 &                               0.2 &                            7.1 &                 2.6 &                          4.7 &                  1.2 \\
\midrule
 Mean &  5.7 & 5.6 & 5.6 & 6.1 & 9.1 & 9.5 & 6.4 & 6.6 \\
 Median &  4.5 & 4.2 &  4.2 & 4.9 & 7.8 & 8.4 & 6.0 & 4.8 \\
\bottomrule
\end{tabular}
